Optimization of the Oktay-Kronfeld Action Conjugate Gradient Inverter

Improving the Fermilab action to third order in heavy quark effective theory yields the Oktay-Kronfeld action, a promising candidate for precise calculations of the spectra of heavy quark systems and weak matrix elements relevant to searches for new physics. We have optimized the bi-stabilized conjugate gradient inverter in the SciDAC QOPQDP library and are developing a GPU code. The action is rewritten and the needed gauge-link combinations are precalculated. In tests with a MILC coarse lattice, this procedure accelerates the inverter by a factor of four. The remaining floating-point operations are mostly simple matrix multiplications between gauge links and fermion vectors, which we accelerate by more than an order of magnitude by using CUDA. Further gains could be achieved by using QUDA.

==> bilinears.tex <==
% Number of bBlinears in the OK action
\begin{table}[!t]
  \footnotesize 
  \tabcolsep 3pt
  \centering
  \renewcommand{\arraystretch}{1.2}
  %
  \subfloat[][]{
    \begin{tabular}{c|C{0.65cm}|C{0.65cm}|C{0.65cm}|C{0.65cm}}
    \hline\hline
    \multicolumn{1}{c}{$d$}&
    \multicolumn{1}{|c}{$4$}&
    \multicolumn{1}{|c}{$5$}&
    \multicolumn{1}{|c}{$6$}&
    \multicolumn{1}{|c}{$7$}\\[0.2ex]
    \hline\hline
    $\lambda^{0}$& $1$&    & & \\ \hline
    $\lambda^{1}$& $1$& $3$& & \\ \hline
    $\lambda^{2}$&    & $1$& $2({\color{BrickRed}0})$& \\ \hline
    $\lambda^{3}$&    &    & $5({\color{BrickRed}4})$& 
    $12({\color{BrickRed}2})$ \\ \hline
    \end{tabular}
    %\caption*{HQET}
    \label{table:sort_bilin_HQET}
  }
  \qquad
  %
  \subfloat[][]{
    \begin{tabular}{c|C{0.65cm}|C{0.65cm}|C{0.65cm}|C{0.65cm}}
    \hline\hline
    \multicolumn{1}{c}{$d$}&
    \multicolumn{1}{|c}{$4$}&
    \multicolumn{1}{|c}{$5$}&
    \multicolumn{1}{|c}{$6$}&
    \multicolumn{1}{|c}{$7$}\\[0.2ex]
    \hline\hline
    $v^{2}$& $2$& $2$& & \\ \hline
    $v^{4}$&    & $2$& $4({\color{BrickRed}2})$&
    $2({\color{BrickRed}1})$  \\ \hline
    $v^{6}$&    &    & $3({\color{BrickRed}2})$&
    $8({\color{BrickRed}1})$  \\ \hline
    $v^{8}$&    &    &       & $2({\color{BrickRed}0})$ \\ \hline
    \end{tabular}
    %\caption*{NRQCD}
    \label{table:sort_bilin_NRQCD}
  }
  %
  \caption{Number of Bilinears}
  \label{table:bilinears}
\end{table}


==> memusage.tex <==
\begin{table}[tb]
  \footnotesize 
  \tabcolsep 3pt
  \centering
  \renewcommand{\arraystretch}{1.2}
  \resizebox{.6\textwidth}{!}{
    \begin{tabular}{c|r|r|r|r|r|r}
    \hline\hline
    \multicolumn{1}{c}{nodes}&
    \multicolumn{1}{|c}{nx}&
    \multicolumn{1}{|c}{ny}&
    \multicolumn{1}{|c}{nz}&
    \multicolumn{1}{|c}{nt}&
    \multicolumn{1}{|c}{CPU(GBytes/node)}&
    \multicolumn{1}{|c}{GPU(GBytes/node)}\\[0.2ex]
    \hline\hline
      4& 20& 20& 20&  64& 1.837& 0.704\\ \hline
     12& 28& 28& 28&  96& 2.520& 0.966\\ \hline
     32& 40& 40& 40&  96& 2.755& 1.056 \\ \hline
     64& 48& 48& 48& 144& 3.571& 1.368\\ \hline
    192& 64& 64& 64& 192& 3.762& 1.441\\ \hline\hline
    \end{tabular}
  }
  \caption{Memory requirements: The first column shows the minimum required 
    nodes to use the OK action CG inverter with the GTX480.}
  \label{table:memusage}
\end{table}


==> timing.tex <==
\begin{table}[bt]
  \footnotesize 
  \tabcolsep 3pt
  \centering
  \renewcommand{\arraystretch}{1.2}
  \resizebox{.4\textwidth}{!}{
    \begin{tabular}{l|r|r}
    \hline\hline
    \multicolumn{1}{c}{Timing~(s)}&
    \multicolumn{1}{|c}{Optimized}&
    \multicolumn{1}{|c}{CUDA}\\[0.2ex]
    \hline\hline
    %Matrix Multiplication~[ALL]& 2579.1& 287.0\\ \hline
    %Matrix Multiplication~[SP]& 2469.3& 241.3\\ \hline
    Matrix Multiplication~[SP]& 2469.3& 79.7\\ \hline
    %Matrix Multiplication~[DP]&  109.7&  45.7\\ \hline
    Matrix Multiplication~[DP]&  109.7&  10.1\\ \hline
    FLOPS~(GF/Nodes)& {\color{BrickRed}2.1}& {\color{BrickRed}58.8}\\
    \hline\hline
    CUDA Memory Copy, $W$& & 44.1\\ \hline
    CUDA Memory Copy, $\psi$& & 191.6\\ \hline
    FLOPS~(GF/Nodes)&    & {\color{BrickRed}18.4}\\ \hline\hline
    QOPQDP Preparation& & 138.9\\ \hline\hline
    Precalculation& \multicolumn{2}{c}{67.1}\\ \hline
    Communication& \multicolumn{2}{c}{7.3}\\ \hline
    Gamma Basis Change& \multicolumn{2}{c}{45.2}\\ \hline
    Spin Decomposition& \multicolumn{2}{c}{62.5}\\ \hline\hline
    \end{tabular}
  }
  \caption{Timing}
  \label{table:timing}
\end{table}

